DecentNeRFs: Decentralized Neural Radiance Fields from Crowdsourced Images

Neural radiance fields (NeRFs) show potential for transforming images captured worldwide into immersive 3D visual experiences. However, most of this captured visual data remains siloed in our camera rolls as these images contain personal details. Even if made public, the problem of learning 3D representations of billions of scenes captured daily in a centralized manner is computationally intractable. Our approach, DecentNeRF, is the first attempt at decentralized, crowd-sourced NeRFs that require $\sim 10^4\times$ less server computing for a scene than a centralized approach. Instead of sending the raw data, our approach requires users to send a 3D representation, distributing the high computation cost of training centralized NeRFs between the users. It learns photorealistic scene representations by decomposing users' 3D views into personal and global NeRFs and a novel optimally weighted aggregation of only the latter. We validate the advantage of our approach to learn NeRFs with photorealism and minimal server computation cost on structured synthetic and real-world photo tourism datasets. We further analyze how secure aggregation of global NeRFs in DecentNeRF minimizes the undesired reconstruction of personal content by the server.

==> algorithms/panda2e.tex <==


\begin{algorithm}[H]
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\SetKwInOut{Require}{require}
\SetKwInput{KwData}{Hyperparameters}
\SetKwFor{For}{for}{do}{end for}

\KwData{Variance $\alpha$, Number of merge rounds $M$, Number of training iterations per merge $\Gamma$}
$\theta^{(0)} \gets \{W^{(0)}, \beta^{(0)}\}$ are initial NeRF weights\;
$L^{(0)}, R \gets \text{Reparameterise}(W^{(0)}, \alpha)$ \tcc*[r]{these are the learnable and frozen parameters; see Sec. 5.2}
$C^{(0)} \gets \{L^{(0)}, \beta^{(0)}\}$\;
Distribute $R$ to all clients $k = 1, \ldots, K$ *\;
\For{client $k = 1$ \KwTo $K$ \tcc*[r]{parallel loop}}{
    $D_k \gets$ data collected by client $k$\;
}
\For{merge round $m = 1$ \KwTo $M$}{
    \For{client $k = 1$ \KwTo $K$ \tcc*[r]{parallel loop}}{
        $C^{(m-1)}$ is received from the server *\;
        $C_k^{(m)} \gets \text{STrain-NeRF}(C^{(m-1)}, R, D_k, \Gamma)$\;
        $C_k^{(m)}$ contains $L_k^{(m)}, \beta_k^{(m)}$; \tcc*[r]{see Sec. 5.2}
        $C_k^{(m)}$ is transmitted to the server *\;
    }
    \For{$k = 1$ \KwTo $K$}{
        $W_k^{(m)} \gets \text{Recover}(L_k^{(m)}, R)$ \tcc*[r]{see Sec. 5.2}
        $\theta_k^{(m)} \gets \{W_k^{(m)}, \beta_k^{(m)}\}$\;
    }
    $\theta^{(m)} \gets \text{Combine}(\{\theta_k^{(m)}\}_{k=1,\ldots,K})$ \tcc*[r]{federated averaging; see Sec. 5.1}
    $L^{(m)} \gets \text{Refactorise}(W^{(m)}, R)$ \tcc*[r]{extract learnable parameters; see Sec. 5.2}
    $C^{(m)} \gets \{L^{(m)}, \beta^{(m)}\}$\;
}
\Output{$\theta^{(M)}$}
\caption{Proposed FedNeRF for the application scenario. Data transfers are marked by *.}
\end{algorithm}


==> algorithms/panda_algo.tex <==
% \begin{algorithm}
% \caption{Proposed PANDA algorithm for K clients. Data transfers are marked by \textcolor{blue}{*}.\zt{fix naming convention, random initialiation of wts, add in parallel and secure compute, refer to sections}}
% \label{alg:panda}
% \begin{algorithmic}[1]
% \REQUIRE Hyperparameters: Weigthed Averaging Learning Rate $\eta$, Number of merge rounds $M$, Number of training epochs per merge $\Gamma$
% \STATE $\{\sigma^{(0)}, \rho^{(0)}\}$ are initial Shared and Public MLP weights
% \STATE $\alpha^{(0)} \rightarrow \{\alpha_1,\alpha_2,\ldots,\alpha_K\}$ are initial client contributions
% \STATE Distribute $\{\sigma^{(0)}, \rho^{(0)}\}$ to all clients $k = 1, \ldots, K$ \textcolor{blue}{*}
% \FOR{merge round $m = 1$ to $M$}
%     \FOR{client $k = 1$ to $K$} %\COMMENT{parallel loop}
%         \STATE $\sigma^{(m-1)}$ is received from the server \textcolor{blue}{*}
%         \IF {$m=1$}
%             \STATE $\rho^{(m-1)}$ is received from the server \textcolor{blue}{*}
%         \ENDIF
%         \IF{$m > 1$}
%             \STATE freeze $\{\sigma_k^{(m-1)}, \rho_k^{(m-1)}\}$
%             \STATE $\frac{\partial L_k^{D}}{\partial \sigma_k^{(m-1)}} \leftarrow \text{\emph{Calc. Gradients}}$
%             \STATE $\left\{\frac{\partial L_k^{D}}{\partial \sigma_k^{(m-1)}}, \sigma_k^{(m-1)}\right\}$ is transmitted to the server \textcolor{blue}{*}
%         \ENDIF
%         \STATE $\{\sigma_k^{(m)}, \rho_k^{(m)}\} \leftarrow \text{NeRF Update}(\sigma_k^{(m-1)}, \rho_k^{(m-1)}, \Gamma)$
%         \STATE $\sigma_k^{(m)}$ is transmitted to the server \textcolor{blue}{*}
%     \ENDFOR
%     \IF{$m > 1$}
%         \STATE $\alpha^{(m)} \leftarrow \text{Alpha Update}(\left\{\frac{\partial L_k^{D}}{\partial \sigma_k^{(m-1)}}, \sigma_k^{(m-1)},\eta\right\})$ %refer to section
%     \ENDIF
%     \STATE $\sigma^{(m)} \leftarrow \text{Secure Aggregation}(\alpha^{(m)},\{\sigma_{k=1,\ldots,K}^{(m)}\})$
%     \STATE $\sigma^{(m)}$ is transmitted to the clients \textcolor{blue}{*}
% \ENDFOR
% \RETURN $\sigma^{(M)}$
% \end{algorithmic}
% \end{algorithm}

\begin{algorithm}
\caption{DecentNeRF algorithm. Data transfers are marked by \textcolor{blue}{*}.\zt{fix naming convention, random initialization of wts, add in parallel and secure compute, refer to sections}}
\label{alg:panda}
\begin{algorithmic}[1]
\REQUIRE Hyperparameters: \\
Weighted Averaging Learning Rate $\eta$, \\
Number of merge rounds $M$, \\
Number of training epochs per merge $\Gamma$.
\STATE $\{g^{(0)}, p^{(0)}\}$ are initial Shared and Public MLP weights
\STATE $\alpha^{(0)} \rightarrow \{\alpha_1,\alpha_2,\ldots,\alpha_K\}$ are initial client contributions
\STATE Distribute $\{g^{(0)}, p^{(0)}\}$ to all clients $k = 1, \ldots, K$ \textcolor{blue}{*}
\FOR{merge round $m = 1$ to $M$}
    \FOR{client $k = 1$ to $K$ in Parallel}  %\COMMENT{parallel loop}
        \STATE $g^{(m-1)}$ is received from the server \textcolor{blue}{*}
        % \IF {$m=1$}
        %     \STATE $p^{(m-1)}$ is received from the server \textcolor{blue}{*}
        % \ENDIF
        \IF{$m > 1$}
            \STATE freeze $\{g_k^{(m-1)}, p_k^{(m-1)}\}$
            \STATE $\frac{\partial L_k}{\partial g_k^{(m-1)}} \leftarrow \text{\emph{Calc. Gradients}}$
            \STATE $\frac{\partial L_k}{\partial g_k^{(m-1)}}$ transmitted to the server \textcolor{blue}{*}
            \STATE $\sum \frac{\partial L_k}{\partial \mathbf{g}^{(m-1)}}$ is recieved from the server \textcolor{blue}{*}
            \STATE $\alpha_k^{(m)} \leftarrow \text{Alpha Update}(\left\{\frac{\partial L_k}{\partial g_k^{(m-1)}}, g_k^{(m-1)},\eta\right\})$
        \ENDIF
        \STATE $\{g_k^{(m)}, p_k^{(m)}\} \leftarrow \text{NeRF}(g_k^{(m-1)}, p_k^{(m-1)}, \Gamma)$
        \STATE $\alpha_k^{(m)} \times g_k^{(m)}$ is transmitted to the server \textcolor{blue}{*}
    \ENDFOR

    \FOR{ server in Parallel }
   
        \STATE $g^{(m)} \leftarrow \text{Secure Aggregation}( \{ \alpha_k \times g_k \} _{k=1,\ldots,K}^{(m)})$
        \STATE $g^{(m)}$ is transmitted to the clients \textcolor{blue}{*}
        \STATE $\sum \frac{\partial L_k}{\partial \mathbf{g}^{(m-1)}} \leftarrow \text{Secure Aggregation}(\{ \frac{\partial L_k}{\partial g_k^{(m-1)}}\}_{k=1,\ldots,K})$
        \STATE  $\sum \frac{\partial L_k}{\partial \mathbf{g}^{(m-1)}}$ is transmitted to the clients \textcolor{blue}{*}        
    \ENDFOR
\ENDFOR
\RETURN $g^{(M)}$
\end{algorithmic}
\end{algorithm}

% g_{k=1,\ldots,K}^{(m)

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> tables/1_blender_baseline/4_blender.tex <==


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|ccc|cc|ccc|cc}
%      & \multicolumn{5}{|c|}{Lego} & \multicolumn{5}{|c|}{Ship} \\
%      \hline 
     
%      & PSNR \uparrow &  SSIM \uparrow & LPIPS \downarrow 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:blender_baseline}
% \end{table}

% ---- dump google sheet copy/paste here
% \begin{scontents}[write-out=data.csv]
% 	Lego					Ship				
% 	Utility			Privacy	Decentralization	Utility			Privacy	Decentralization 
% 	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	PSNR\downarrow SSIM\uparrow	Server (Flops)\downarrow PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	SSIM\downarrow	Server FLOPs\downarrow
% NeRF-W \cite{martin2021nerf}	\textcolor{blue}{27.09}	\textcolor{blue}{0.934}	\textcolor{blue}{0.0513}	0	20 M	\textcolor{blue}{26.35}	\textcolor{blue}{0.8661}	\textcolor{blue}{0.1765}	1	20 M
% FedNeRF \cite{holden2023federated}	17.7	0.858	0.2003	\textcolor{BurntOrange}{0.08}	\textcolor{blue}{1K}	20.92	0.8281	0.2368	\textcolor{BurntOrange}{0.92}	\textcolor{blue}{1K}
% PANDA (ours)	\textcolor{BurntOrange}{26.25}	\textcolor{BurntOrange}{0.92}	\textcolor{BurntOrange}{0.0652}	\textcolor{blue}{0.2}	\textcolor{BurntOrange}{10K}	\textcolor{BurntOrange}{24.58}	\textcolor{BurntOrange}{0.8554}	\textcolor{BurntOrange}{0.1901}	\textcolor{blue}{0.23}	\textcolor{BurntOrange}{10K}
% \end{scontents}


\begin{scontents}[write-out=data.csv]
	Lego						Ship					
	Utility			Privacy		Decentralization	Utility			Privacy		Decentralization
	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	PSNR\downarrow	SSIM\downarrow	Server FLOPs\downarrow	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	PSNR\downarrow	SSIM\downarrow	Server FLOPs\downarrow
NeRF-W 	\textcolor{Blue}{27.09}	\textcolor{Blue}{0.934}	\textcolor{Blue}{0.0513}	\infty	0	130 T	\textcolor{Blue}{26.35}	\textcolor{Blue}{0.8661}	\textcolor{Blue}{0.1765}	\infty	0	$\approx$ 220T
FedNeRF	17.7	0.858	0.2003	26.06	0.81	0.6 B	20.92	0.8281	0.2368	27.21	0.82	$\approx$ 1 B
PANDA 	\textcolor{BurntOrange}{26.25}	\textcolor{BurntOrange}{0.92}	\textcolor{BurntOrange}{0.0652}	14.59	0.62	4.8 B	\textcolor{BurntOrange}{24.58}	\textcolor{BurntOrange}{0.8554}	\textcolor{BurntOrange}{0.1901}	13.79	0.61	$\approx$ 8 B
\end{scontents}






% NeRF-W (centralized privacy-agnostic) FedNeRF (decentralized privacy-agnostic) PANDA (decentralized privacy-aware)


\begin{table*}[ht]
\centering 
\scalebox{0.77}{{\begin{tabularx}{\textwidth}{l|ccc|cc|c|ccc|cc|c}
\input{|python script.py}
\end{tabularx}}}
\caption{\textbf{Quantitative results on Private Blender dataset}:
Best and second best results for utility are highlighted in blue and orange respectively. A privacy-agnostic centralized approach \cite{martin2021nerf} achieves the best utility performance while using ~\textbf{$10^5$} more server compute than other approaches. FedNerf \cite{holden2023federated} even though it only is 8x server compute cheaper than PANDA and performs poorly on utility metrics and leaks out the most private details as reference by the high SSIM an PSNR numbers. In contrast, PANDA obtains comparable utility to centralized approaches, is the most private, and has server computation several orders of magnitude lower than the centralized approach. Number of training rounds is different for FedNeRF and PANDA. }
\end{table*}





==> tables/1_comparison.tex <==
\begin{table}
    \centering
    \footnotesize
    \begin{tabular}{lccccc}
        \toprule
        \textbf{Approach} & \textbf{Utility} & \textbf{Privacy} & \multirow{2}{*}{\textbf{Data Transfer}} & \multirow{2}{*}{\textbf{Server Compute}} & \multirow{2}{*}{\textbf{Client Compute}} \\
        \midrule
        \textbf{NeRF-W} & \textcolor{green}{High} & \textcolor{red}{None} & \textcolor{green}{\checkmark} & High & None \\
        \textbf{FedNeRF} & Low & High & Low & Low & High \\
        \textbf{PANDA(ours)} & High & High & Low & Low & High \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of different methods.}
    \label{tab:comparison}
\end{table}

==> tables/2_phototourism_baseline/photo_baseline.tex <==


% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|ccc|cc|ccc|cc}
%      & \multicolumn{5}{|c|}{Lego} & \multicolumn{5}{|c|}{Ship} \\
%      \hline 
     
%      & PSNR \uparrow &  SSIM \uparrow & LPIPS \downarrow 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:blender_baseline}
% \end{table}

% ---- dump google sheet copy/paste here
\begin{scontents}[write-out=data2.csv]
	Bradenburg Gate			Trevi Fountain			Sacre Coeur		
	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow	PSNR\uparrow	SSIM\uparrow	LPIPS\downarrow
NeRF-W \cite{martin2021nerf}	\textcolor{blue}{25.18}	\textcolor{blue}{0.901}	\textcolor{blue}{0.1927}	\textcolor{blue}{21.49}	\textcolor{blue}{0.7206}	\textcolor{blue}{0.2866}	\textcolor{blue}{20.58}	\textcolor{blue}{0.7835}	\textcolor{blue}{0.2305}
FedNeRF \cite{holden2023federated}	18.92	0.8158	0.3528	16.55	0.5774	0.4352	15.41	0.6555	0.4072
PANDA(A)	23.61	0.8535	0.329	20.04	0.6439	0.5261	18.82	0.6777	0.3874
PANDA	\textcolor{BurntOrange}{24.62}	\textcolor{BurntOrange}{0.8802}	\textcolor{BurntOrange}{0.2571}	\textcolor{BurntOrange}{20.61}	\textcolor{BurntOrange}{0.6501}	\textcolor{BurntOrange}{0.3963	} \textcolor{BurntOrange}{19.22}	\textcolor{BurntOrange}{0.7259}	\textcolor{BurntOrange}{0.3126}
\end{scontents}



\begin{table*}[h!]
\centering
\label{tab:photo_qual}
%\resizebox{\linewidth}{!}
{\scalebox{0.74}{\begin{tabularx}{\textwidth}{l|ccc|ccc|ccc}
\input{|python script.py}
\end{tabularx}}}
\caption{\textbf{Quantitative reconstruction performance on Phototoursim dataset\cite{snavely2006photo} for NeRF-W, FedNeRF, and PANDA ablations}: Best and second best results are highlighted in blue and orange respectively. As expected, privacy-agnostic centralized NeRF-W \cite{martin2021nerf} performs best across all metrics, followed closely by PANDA. This demonstrates our privacy-aware decentralized approach (PANDA) is effective for real-world datasets compared to other privacy-agnostic decentralized approaches \cite{holden2023federated} }
\end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{|l|lll|lll|lll|}
% \hline
% Method   & \multicolumn{3}{c|}{Bradenberg Gate}                & \multicolumn{3}{c|}{Trevi Fountain}                 & \multicolumn{3}{c|}{Sacre Coeur}                    \\ \hline
%  &
%   \multicolumn{1}{l|}{PSNR} &
%   \multicolumn{1}{l|}{SSIM} &
%   LPIPS &
%   \multicolumn{1}{l|}{PSNR} &
%   \multicolumn{1}{l|}{SSIM} &
%   LPIPS &
%   \multicolumn{1}{l|}{PSNR} &
%   \multicolumn{1}{l|}{SSIM} &
%   LPIPS \\ \cline{2-10} 
% NeRF-W   & \multicolumn{1}{l|}{1} & \multicolumn{1}{l|}{1} & 2 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 \\
% FedNeRF  & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{1} & 2 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 \\
% PANDA(A) & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{1} & 2 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 \\
% PANDA    & \multicolumn{1}{l|}{3} & \multicolumn{1}{l|}{1} & 2 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3 & \multicolumn{1}{l|}{2} & \multicolumn{1}{l|}{3} & 3\\
% \hline
% \end{tabular}
% \end{table*}



==> trash/1_intro.tex <==
\section{Introduction}
\label{sec:intro}





%-------------------------------------------------------------------------
With the advent of digital cameras, capturing images has become an integral part of daily life. People effortlessly take photos in a variety of settings, ranging from restaurants, bars, and coffee shops, to iconic monuments, bustling streets, and the intimate spaces of their homes. Of the hundreds of images stored on people's phones only a mere fraction reach the public domain. Leveraging this substantial repository of private visual data silos, this paper endeavors to generate 3D scene renderings that transcend the limitations imposed by the sole reliance on publicly available data.

\zt{applications: concertnerf, virtual tours, photo-tourism}

The traditional method of deploying agents to collect data for the generation and continual updating of NeRF models \cite{GoogleNERF2023} of "every corner of the world" is subject to inherent limitations in terms of scalability, cost, and efficiency. While the approach to crowdsource user data can overcome these limitations, it presents two additional challenges. Secondly, because of the sensitive nature of private user data, transferring data to a central server has serious privacy implications.

To overcome these scalability and privacy issues we propose learning the NeRF models in a decentralized manner leveraging the recent advances in Federated Learning \cite{kairouz2021advances} and secure aggregration\cite{burkhart2010sepia}. A key insight of our approach is that crowdsourced images are comprised of scene-specific elements consistent across different clients in terms of 3D structure and texture for a specific scene, and client-specific elements that are semantically private, such as people, sensitive objects, and text. Therefore, we use a NeRF architecture which is a composite of two Multi-Layer Perceptrons (MLPs) \cite{martin2021nerf}, a Public Scene MLP, and a Client Specific MLP able to decompose these two elements of the images. Further, we only share the weights of Public Scene MLP with the server using Multi-Party Computation(MPC) \cite{burkhart2010sepia} protocol of secure aggregation to make sure an untrusted server only ever accesses the averaged model. Deviating, from the standard federated learning practice of weighted averaging of client models proportional to the number of samples (number of pixels) on that client, we propose an end-to-end pipeline to optimize every client's contribution to the global server model to account for the disparity of views that clients would have in a crowd-sourced setting. This decentralized learning approach which we name PANDA, provides reconstruction performance parity with a centralized approach while providing the highest privacy guarantees.

While previous attempts at Federated Learning of NeRFs have made insightful contributions in terms of model compression to optimize communication bandwidth costs \cite{holden2023federated} and facilitating large-scale scene modeling \cite{suzuki2023federated}, these attempts have not fully encapsulated the complexity and "real-worldness" of unconstrained crowdsourced imagery \cite{snavely2006photo}. The underlying assumption in prior works is a scenario wherein every element within the scene remains static and is non-private, while the scene is simultaneously captured by all participating clients. We show in \ref{privacy_average} that when dealing with crowd-sourced data these approaches not only leak private information without a secure aggregation protocol but also result in inaccurate reconstructions on the server. 

To quantify these privacy-utility trade-offs we introduce a benchmark dataset of blender simulations of scenes comprising both scene-specific and private elements varying across clients and establish specific evaluation protocols. This is complemented by evaluations on real-world crowd-sourced images \cite{snavely2006photo}. Finally, we demonstrate that initializing the clients with a model trained centrally on limited auxiliary public data \cite{ji2014differential} (i.e. free of privacy concerns) which by itself gives poor reconstruction quality, can accelerate the convergence of our PANDA approach.

To summarize, we make the following contributions:

\begin{itemize}
    \item We present PANDA, our approach of locally training a split NeRF model, and then securely aggregating the Public Scene MLPs from different clients while keeping the Client Specific MLP that implicitly captures semantically private information local to the clients.
    \item We introduce a smart averaging approach that learns the optimal contribution of each client to the global scene MLP model in an end-to-end fashion to account for the richness of data in terms of view disparity across clients. This approach achieves the highest reconstruction performance in terms of PSNR and SSIM among all decentralized approaches. 
    \item We introduce a simulated dataset and empirical privacy evaluation metrics that serve as a benchmark for future work in the space of privacy-aware 3D rendering using crowd-sourced data.
    \item We demonstrate that having limited auxiliary public data can accelerate the convergence of our approach.
    \item \zt{we are the first }

\end{itemize}

\zt{Think more about Limitations}
\zt{A paragraph clarifying privacy guarantees provided by our work, discussing MI attacks and suggesting DP methods can be easily integrated to provide formal guarantees that can be left for future work }

List of Figures and Tables
\begin{enumerate}
    \item Fig1 Teaser Figure talking about crowd-sourced images, our approach and data
    \item Table1 comparing baselines with us on a high level
    \item Fig2 Describing the PANDA approacch
    \item Fig3 Describing averaging using an image and rays
    \item Algorithm: Psuedo-Code
    \item Table2 Results for Ablations on Blender
    \item Table2a/Figure Smart aggregation case
    \item Fig4 Results on Blender Scenes
    \item Fig 5 Smart averaging
    \item Table3 Public Private 
    \item Table 4 phototourism scenes
    \item Fig6 phototourism closeups`            


    \item (Supp) generation of blender data and masks
    \item (Supp) vary number of clients
    \item (Supp) vary public/private split
    \item (Supp) Privacy Utility leakage over rounds
    \item (Supp) Membership Inference
    \item (Supp) fig4a client views for fednerf and panda for blender
    \item (Supp) fig5a client views for fednerf and panda for phototourism
    
\end{enumerate}

\zt{
Paragraph 1. What is the problem/vision (intention)? WHy is it important (stakes)? Motivate with multiple examples
    a. Crowd-sourced NeRF
    b. Harnessing wealth of data people already have on their camera rolls
    c. No need to explicitly capture a scene by a single person.
2. What are key challenges in realizing this vision? (constraints) Could be motivated with a single example
   a. The amount of data:
      I. Both for a single scene and for multiple scenes
      II.  Computationally impractical to dump all of this on a single server 
    b. Data is private:
      I. Even if a is solved, people won't be willing to share private data
3. What is your key insight and how you would tackle the challenges? (mini - contribution)
   a. Decentralized + Privacy
   b. Demonstrate results with high utility and high privacy on variety of datasets. (number to back it up)
4. How what you are doing is different / improves upon prior works
5. Our approach:
6. Contributions
7. Limitations
}


% 6. Contributions
% \begin{itemize}
%     \item Crowdsourced NeRFs using decentralized learning for Unconstrained Image Collections giving optimal Privacy and Utility Performance
%     \item Smart Averaging 
%     \item Public model to help with 
%     \item Deal with the single image case
%     \item Provide a dataset and methodology to quantify privacy utility trade-offs of different approaches
% \end{itemize}

% 7. Limitations




==> trash/1_intro_v2.tex <==




\section{Introduction}
\label{sec:intro}

% Pass 3: Akshat

% AD: Outline Next Pass
% 1. Motivation
%    - What is the problem you are solving (intention)
%    - Why is it important 
% 2. What are the key challenges in realizing this vision
%    - Decentralization 
%    - Privacy
% 3. What is your key insight and how you would tackle the challenges ? 
% 4. How what you are doing is different / improves upon prior works.
% 5. Our Approach 
% 6. Our contributions.
% 7. Scope.


%-------------------------------------------------------------------------
% Pass 2: Kush 
Imagine exploring Machu Picchu in Peru, where every trekker's photos of hidden nooks, terraces, and stone pathways combine to generate a 3D map, revealing the ancient city's layout in unparalleled detail. Yet, such a detailed 3D reconstruction of the scene remains infeasible due to three challenges: 1) the images on tourist devices often contain sensitive and personal information and, therefore, cannot be used directly 2) such images are stored in a decentralized fashion across users' devices which presents a challenge to 3D modeling algorithms which are typically centralized, and 3) the images are often captured in-the-wild and contain variable illumination, angles, and occlusions that presents a challenge for 3D modeling algorithms. Our aim is to enable crowd-sourced 3D modeling in a private, scalable, and decentralized fashion. 

To overcome these challenges, we propose a semantically private, in-the-wild, and decentralized way to learn Neural Radiance Fields. Our approach uses geo-tagged, decentralized, and private images of a certain scene held in client devices to learn \textit{Public} and \textit{Private} Radiance Fields. The \textit{Public} Field is learned by aggregating the \textit{semantically-public pixels} that are present in user images, which can then be queried to perform 3D reconstruction of the public aspects of the scene. This radiance field formulation of 3D reconstruction by triangulating rays per pixel from different views lends itself well to this problem as the public pixels viewing similar parts of the scene can be triangulated across the diverse set of client views in a secure manner. Additionally, as a consequence of learning a \textit{Public} Radiance Field across clients, we also learn a client-specific, on-device \textit{Private} Radiance Field using all pixels that are not classified as \textit{public} i.e. semantically-private pixels. Learning \textit{Public} Radiance Fields across clients also improves the 3D reconstruction of private parts of the image such as people in a 3D scene. Moreover, our \textit{Public} and \textit{Private} Radiance Field approach also enables each client to render novel views of themselves in the scene from any of the client views present in the scene. 


\kt{paragraph about how the process is done so did a pass, but not sure how to write it need to know exactly what's happening.. this paragraph is about the nerf side of things } We first decompose the image into public and private pixels for each client \kt{not sure if this is done anymore}. Then for all the public pixels, we train a Public MLP that is shared across all clients. At the same time, the client also contains a private MLP that is responsible for learning all the private and transient features in the scene. We label all the parts of the scene that are globally transient (parts of the scene that are transient across images from all clients) in an image as private. 

\kt{paragraph about how the process is done so did a pass, but not sure how to write it need to know exactly what's happening.. this paragraph is about the FEDLEARNIGN side of things} Once the scene is divided, we aggregate the 3D features securely from each client's public MLP using secure multiparty computation (MPC). However, when averaging Public Radiance Fields, each client doesn't have the same contribution as some clients might have redundant and non-unique views which leads to overfitting to a specific client's public data. To alleviate this issue of view distribution across clients, we propose a Smart Averaging for View Discrepancy method that learns the optimal contribution of each client to the global scene MLP. This approach achieves the highest reconstruction performance in terms of PSNR and SSIM among all decentralized approaches. 

Similar to other approaches in the field \kt{citeme}, our approach also lies on a privacy-utility tradeoff curve. We analyze this tradeoff and its effect on Crowd-Sourced, Private, and Decentralized Neural Rendering. We introduce a benchmark dataset of blender simulations of scenes comprising both scene-specific and private elements varying across clients and establish specific evaluation protocols. This is complemented by evaluations on real-world crowd-sourced images \cite{snavely2006photo}. Finally, we demonstrate that initializing the clients with a model trained centrally on limited auxiliary public data \cite{ji2014differential} (i.e. free of privacy concerns) which gives poor reconstruction quality, can accelerate the convergence of our PANDA approach.

% While previous attempts at Federated Learning of NeRFs have made insightful contributions in terms of model compression to optimize communication bandwidth costs \cite{holden2023federated} and facilitating large-scale scene modeling \cite{suzuki2023federated}, these attempts have not fully encapsulated the complexity and "real-worldness" of unconstrained crowdsourced imagery \cite{snavely2006photo}. The underlying assumption in prior works is a scenario wherein every element within the scene remains static and is non-private, while the scene is simultaneously captured by all participating clients. We show in \ref{privacy_average} that when dealing with crowd-sourced data these approaches not only leak private information without a secure aggregation protocol but also result in inaccurate reconstructions on the server. 

To summarize, we make the following contributions:

\begin{itemize}
\item We present a method to train Neural Radiance Fields for a large-scale, decentralized, and private setup by learning Public Radiance Field that is trained across clients on a Server, and Private Radiance Fields that is trained on-device. 
    \item We learn our Public and Private Radiance Fields to implicitly capture semantically private information local to the clients and globally transient to all clients viewing the scene.  
    % to locally train a split NeRF model, and securely aggregate the Public Scene MLPs from different clients while keeping the Client Specific MLP that 
    
    \item We introduce a smart averaging approach to alleviating the view distribution problem across clients that results in the best reconstruction performance among decentralized approaches 
    
    \item We provide insights on the privacy-utility tradeoff when training Neural Radiance Fields as a function of its inputs: view distribution, number of clients, and \kt{somethign else}. 
    
    \item We introduce a simulated dataset and empirical privacy evaluation metrics that serve as a benchmark for future work in the space of privacy-aware 3D rendering using crowd-sourced data.
    
    \item We demonstrate that having limited auxiliary public data can accelerate the convergence of our approach.
    
    \item \zt{we are the first }

\end{itemize}

\textbf{Scope.} Our work assumes that privacy is transient \kt{put stuff here.. }
% \zt{Think more about Limitations}
% \zt{A paragraph clarifying privacy guarantees provided by our work, discussing MI attacks and suggesting DP methods can be easily integrated to provide formal guarantees that can be left for future work }

% List of Figures and Tables
% \begin{enumerate}
%     \item Fig1 Teaser Figure talking about crowd-sourced images, our approach and data
%     \item Table1 comparing baselines with us on a high level
%     \item Fig2 Describing the PANDA approacch
%     \item Fig3 Describing averaging using an image and rays
%     \item Algorithm: Psuedo-Code
%     \item Table2 Results for Ablations on Blender
%     \item Table2a/Figure Smart aggregation casezz
%     \item Fig4 Results on Blender Scenes
%     \item Fig5 Privacy Leakage over rounds 
%     \item Table3 Public Private 
%     \item Table 4 phototourism scenes
%     \item Fig6 phototourism closeups`            


%     \item (Supp) generation of blender data and masks
    
% \end{enumerate}


% \zt{
% Paragraph 1. What is the problem/vision (intention)? WHy is it important (stakes)? Motivate with multiple examples
%     a. Crowd-sourced NeRF
%     b. Harnessing wealth of data people already have on their camera rolls
%     c. No need to explicitly capture a scene by a single person.
% 2. What are key challenges in realizing this vision? (constraints) Could be motivated with a single example
%    a. The amount of data:
%       I. Both for a single scene and for multiple scenes
%       II.  Computationally impractical to dump all of this on a single server 
%     b. Data is private:
%       I. Even if a is solved, people won't be willing to share private data
% 3. What is your key insight and how you would tackle the challenges? (mini - contribution)
%    a. Decentralized + Privacy
%    b. Demonstrate results with high utility and high privacy on variety of datasets. (number to back it up)
% 4. How what you are doing is different / improves upon prior works
% 5. Our approach:
% 6. Contributions
% 7. Limitations
% }


% 6. Contributions
% \begin{itemize}
%     \item Crowdsourced NeRFs using decentralized learning for Unconstrained Image Collections giving optimal Privacy and Utility Performance
%     \item Smart Averaging 
%     \item Public model to help with 
%     \item Deal with the single image case
%     \item Provide a dataset and methodology to quantify privacy utility trade-offs of different approaches
% \end{itemize}

% 7. Limitations




==> trash/4_methodology_v1.tex <==
\section{PANDA approach}
For a given scene with \( K \) known users and \( N \) images distributed among them such that individual users have \((n_1, n_2, \dots, n_K)\) images on their device, where \(\sum_{i=1}^{K} n_i = N\). In a naive federated learning approach, \cite{holden2023federated} each user will learn its own volumetric 3D representation on its set of images {$n_k$} using a global MLP ($\sigma_k$) using the NeRF pipeline to share it with the server. 

\textbf{Known Camera Pose Assumption}: The NeRF pipeline assumes known, accurate camera poses. In centralized settings, structure from motion (SfM) on image feature descriptors like SIFT can derive relative camera poses using COMLAP \cite{schonberger2016structure}. Decentralized SfM is an active research area, involving sending privatized image feature descriptors to an untrusted server for camera pose estimation. Some methods \cite{speciale2019privacy,dusmanu2021privacy} claim empirical privacy guarantees, while recent work \cite{pittaluga2023ldp} provides formal differential privacy guarantees at a small performance cost. For our purposes, we assume global camera poses are known accurately. While decentralized SfM is still advancing, our method focuses on the complementary problem of decentralized neural radiance fields.

\textbf{Vanilla NeRF backbone \cite{nerf}} At its core, NeRF trains an MLP $\mathbf{sigma_k}$ that takes a 5D input vector: a 3D spatial coordinate $\mathbf{x} = (x, y, z)$ within the scene, and pitch $\theta$ and yaw $\phi$ parameters of the viewing direction $\mathbf{d}$. The MLP outputs a scalar density $\sigma$ and an RGB color vector $\mathbf{c} = (r, g, b)$. 

NeRF rendering synthesizes images via volume rendering, sampling predicted color and density at many points along rays traversing the scene. For, a particular ray corresponding to pixel the MLP predicts a color vector $\mathbf{c} = (r, g, b)$ and compares it with the ground truth RGB value, using the loss to train the MLP $\mathbf{sigma_k}$. We refer the reader to \cite{nerf} and the supplementary \ref{supp:nerf_pipeline} for more details on NeRF. 

%------------------------------------
\subsection{Personal-Global Content Separation}
\label{sec:client_scene_sep}
\input{figures/fig3_method/method}
Instead of each user learning the scene representation using a single MLP $\mathbf{sigma_k}$, we model the scene using global and personal MLPs, as shown in Fig. \ref{fig:method}. As stated, the personal mlp intends to captures sensitive/private content and is kept native to the user device while the global mlp captures shared global content across users via federation. Each MLP outputs its own scalar density $\sigma$ and an RGB color vector $\mathbf{c} = (r, g, b)$, so the rendered image is an alpha-composite of both output images. The composite image lost trains the network to separate global and personal implicitly. Taking a loss wrt to the gt RGB value, this composite image can help train the network in a way so that the global and scene content separates out. Since on every user itself the images can differ in personal content the personal MLP also takes image index number through a vector embedding as an input. So different views produce different personal content. 

Our architecture is inspired by NeRF in the Wild (nerfw) works in \cite{martin2021nerf,chen2022hallucinated}, with each user essentially running NeRF-W locally. The global and personal MLP are analogous to the static and transient MLPs in the context of a single user. However, we feel global-personal definition better suits the decentralized setting since NeRF-W's transient MLP will not separate all of the personal content from the user. Imagine a subject being recorded in front of a monument with multiple images. Since the subject would be static across all views in the user's image it would be still considered static and thus, won't show up in the transient MLP even though it's considered personal (sensitive) content.  Our federation of global MLP across users over multiple rounds would better separate this user-static but personal content into the personal MLP branch.

\textbf{Apperance modeling} Since the images within and across users would have different photometric variations because of lighting changes, camera settings, etc. we model those with an image-dependent appearance embedding input to the global MLP branch. We don't however share this appearance embedding with the server. We would refer the reader to \cite{martin2021nerf} and the supplementary for more details on this.

Unlike some other approaches to visual privacy in vision tasks like action recognition and depth estimation, we do not explicitly define privacy expectations with an adversarial loss, whether supervised \cite{wu2018towards,tasneem2022learning} or self-supervised\cite{dave2022spact}. Such approaches aim to sanitize pre-defined private (personal) content. Approaches like in-painting for NeRF\cite{weder2023removing} also require explicit masks and have only been shown in a centralized setting. In our case, we implicitly define private content as the personal MLP output, with privacy empirically evaluated in Section \ref{sec:results}. This shows our global MLP does not leak users' personal details, making explicit techniques redundant given our global-personal decomposition.

\subsection{Learned weighted averaging}
\label{sec:learned_wts}
The global MLP at any aggregation round $m$, defined as $\sigma^{(m)} = \sum{\alpha_k^m \cdot \sigma_k^m}$. In a naive federated learning approach, all user global MLP $\sigma$ are weighted equally, $\alpha_k= \frac{1}{K}$, while FedAvg would define them as $\alpha_k = \frac{n_k}{n_K}$ for all $k=1,\ldots,K$, where $n_k$ is the number of image pixels on the $k$th user and $\sum_{k=1}^{K} n_k = n_K$, thus weighing the user contribution proportional to the number of pixels each user contains.   

In the context of NeRfs these explicit definitions would lead to suboptimal reconstruction performance as shown in \ref{fig6:smart_aggregation}. The reason is that all users have different data distributions -  number of views, view disparity, client/scene content ratios and would be able to do different levels of global-personal content decomposition to benefit the server's global representation. We aim to learn the $\alpha$ implicitly over different merge rounds by the following equation 

\begin{equation}
\label{eq:iterative_update}
    \alpha_k^{(m)} = \alpha_k^{(m-1)} - \eta \frac{\partial L}{\partial \alpha_k^{(m-1)}}
\end{equation}

where \(\eta\) is the weighted averaging learning rate, and the cumulative loss \(L\) is defined as the sum of losses for each user \(k\), \(L = \sum L_k\), where \(L_k\) is given by

\begin{equation}
    L_k = \text{L2norm}\left| I\left(\sigma^{(m-1)}\right) + \beta I\left(\rho_k^{(m-1)}\right), I(\text{GT})\right|
\end{equation}
\zt{technically its the same as the nerfw loss and should be written like that}
The loss implicitly rewards the users alpha when they  MLPs when they do a better global-personal decomposition. \zt{write it ina better way} Combining the above with the update equation for \(\alpha_k\), w

\begin{equation}
    \frac{\partial L}{\partial \alpha_k}^{(m-1)} = \left( \sum \frac{\partial L_k}{\partial \sigma^{(m-1)}} \right) \cdot \sigma_k^{m-1}
\end{equation}


Beyond merge round 1, each user sends its own \(\frac{\partial L_k}{\partial \sigma^{(m-1}}\), which is aggregated by the server, which gets multiplied with the previous round's client weights (sent again by the users) to update each client's \(\alpha_k\) at every round.

\zt{it should be called iterative updating of weigths}

calculating a loss on the performance of the server global MLP 



\subsection{MPC for secure computation}
% API Spec
\label{sec:mpc}
From the point of view of the users, at every round, there are exactly two kind of messages that each user $k$ communicates with the server - 1) weights of the MLP $\sigma_k$, and 2) gradients with respect to the local loss $\frac{\partial L_k}{\partial \sigma^{(m-1)}_k}$. Due to the previously discussed privacy constraints, we aim to obfuscate these two kinds of messages such that only the final result aggregated over all the users is visible to the server. From the server's perspective, it needs to compute - 3) weighted average of the obfuscated weights sent by the users ($\sigma^{(m)}$), and 4) gradient updates of $\alpha$ ($\frac{\partial L^{(m-1)}}{\partial \alpha_k}$). Each of these four functional requirement is satisfied using secure multi-party computation. We make standard security assumptions as made in the literature such as non-colluding users and honest but curious participants. We now describe the protocols in more detail.

$\mathsf{send\_wts(\sigma^{(m)}_k)}$: Each user obfuscated its local weights by applying a random mask or encrypting data using additively homomorphic encryption techniques. This randomization ensures that when the obfuscated weights are aggregated, the original values can not be recovered from those weights while providing the means to calculate the weighted average accurately.

$\mathsf{weight\_avg({\sigma})}$: This function executes the computation of the weighted average of the obfuscated weights sent by the users ($sigma^(m)$). By employing secure multi-party computation techniques, the server aggregates the masked weights received from all users. There are different trade-offs when choosing the specific multi-party computation technique for this function such as secret key exchange overhead, cross-client communication and synchronization and number of non-colluding servers. Based on the available options for a given system, one can choose an appropriate function and enable the server to obtain the weighted average.

$\mathsf{send\_grads()}$ This function is similar to $\mathsf{send\_wts}$ in its design as each user communicates its local gradients by performing randomized obfuscation to its gradients in a similar way it performs obfuscation of the weights.

$\mathsf{compute\_grads()}$ This function is relatively complex due to the server's computation of $\frac{\partial L^{(m-1)}}{\partial \alpha_k}$ depending upon the product of two obfuscated values - $\frac{\partial L_k}{\partial \sigma^{(m)}}$ and $\sigma^{(m)}_k$. While the sum operations used so far are easy to perform in the encrypted or masked space due to linearity, this time we can not use simple masking based approaches due to the multiplication operation. Therefore, we use beaver triples protocol~\cite{beaver1992efficient} to enable construction of multiplication circuits jointly computed by the users and the server while preserving the privacy constraints. The beaver triples approach imposes additional communication overhead and requires additional synchronization due to pre-processing required in its computation.
% Each user communicates their model weights to the server for aggregation.
% Consider three participants: Alice, Bob, and Charlie, each possessing unique perspectives of a scene. The collective set of their images can be utilized to construct a 3D representation of the scene. However, the challenge is to allow users to contribute their knowledge without exposing their images to others. Therefore, we securely aggregate the model updates from each user, revealing only the aggregated weights to untrusted users. This problem can be addressed using Multi-Party Computation (MPC).

% MPC involves representing information (model updates in our case) as numbers in a finite field ($\mathbb{F}_p$). Each user takes a secret number $x$ and computes $c$ secret shares of $x$ - $r_1$, $r_2$ and $r_3$ where $c$ is the number of users and $r_1 + r_2 + r_3 = x$. A simple approach is to uniformly sample $r_1$ and $r_2$ from the finite field and set $r_3 = x - r_1+r_2$. We denote Alice's shares as $[a]$, where $[a] = [a]_1 + [a]_2 + [a]_3$ and similar notation for others.

% In the secure aggregation protocol, Alice computes $[a]$, Bob computes $[b]$, and Charlie computes $[c]$. Alice shares $[a]_2$ with Bob and $[a]_3$ with Charlie. Bob shares $[b]_2$ with Alice and $[b]_3$ with Charlie. Similarly, Charlie shares $[c]_2$ with Alice and $[c]_3$ with Bob. Each participant locally sums up their shares, shares only the output with the others, and obtains the final sum. Usage of such an additive secret sharing protocol is very efficient in terms of communication and computation and its security guarantees have been well-established\cite{shamir1979share} and requires no collusion between more than $k$ parties where $k$ can be chosen as a system parameter.

% Exploiting the linearity of the average operation, the protocol can be extended to support weighted averaging for our federated learning system. This allows participants \zt{should this be server???} to collectively compute the weighted average of model updates securely. Furthermore, the same protocol can be applied to a set of numbers in a finite field, not just a single number. This enables vectorization of weights in the static Multi-Layer Perceptron (MLP) as a set of integers (modulo $p$) in the finite field, facilitating secure averaging.
% send_wts() | communication | user sends encrypted/masked weights to the server
% weight_avg() | computation | the server averages the weights and obtains the decrypted results
% send_grads() | communication | user sends encrypted/masked gradients to the server
% compute_grads() | computation | the server computes gradients by multiplying the encrypted weights and the encrypted gradients

\subsection{PANDA algorithm}
The key steps of the PANDA algorithm are below accompanied by the pseudo-algorithm in Algo.~\ref{alg:panda}:
\begin{itemize}
    \item Assumes random initialization of global \(\mathbf{G^{(0)}}\) and personal MLP weights \(\mathbf{P^{(0)}}\) at all \(K\) clients.
    \item (On the user) For each round the clients return the current \(\mathbf{G_k^{(m)}}\) and previous rounds global MLP \(\mathbf{G_k^{(m-1)}}\) weights along with loss gradients of previous round global MLP weights \(\frac{\partial L_k}{\partial \mathbf{G}^{(m-1)}}\)
    \item (On the server) For each round the weights are securely aggregated and sent back to the user while the gradients and weights from previous round are used to update user \(\alpha_k\) securely
\end{itemize}


